A Programming, Robotics and Automatic Control Intervention for Secondary Education Students in Sweden and Italy

This study evaluates the AutoSTEM workshop, an intervention for secondary education that combines a serious game with PID-controlled hardware. Seven workshops were conducted across Sweden and Italy. The six Swedish workshops adopted an explicitly SDT-informed facilitation framework, while the Italian workshop followed the existing educational robotics format without a formally defined SDT facilitation protocol. Self-reports, an objective knowledge quiz, and qualitative responses were analysed using multiple site-adjusted statistical approaches. Technical-specific self-efficacy increased substantially in both conditions, with large effect sizes, while objective knowledge showed only modest, non-significant gains. No significant site-adjusted differences were found between SDT and control conditions for the primary outcomes. Perceived engagement was higher in the control condition, although this finding should be interpreted cautiously. The objective knowledge composite remained positive but non-significant across sensitivity analyses. Female participants reported smaller PID self-efficacy gains than males. Qualitative findings supported evidence of PID learning while identifying technical and pacing barriers. Overall, the results suggest that the technology-rich intervention supports competence development, regardless of SDT-informed facilitation.

==> tables/adjusted.tex <==
\begin{table}[t]
\centering\small
\caption{Between-condition difference-in-differences ($\Delta\Delta$ = SDT minus Control change) under three specifications. Unadjusted: pooled pre/post OLS. Covariate-adjusted: adds age, gender and session-composition case-mix covariates (prior robotics, programming, automatic control, simulator use and gaming). Site fixed effects: session dummies absorb all stable site differences, so $\Delta\Delta$ is identified from condition-specific pre--post change. Robust (HC1) standard errors. $^{*}p<0.05$, $^{**}p<0.01$, $^{***}p<0.001$.}
\label{tab:adjusted}
\begin{tabular}{lrrrrr}
\toprule
Outcome & Unadj. & Covariate-adj. [95\% CI] & $p$ & Site FE [95\% CI] & $p$ \\
\midrule
PID self-efficacy (composite) & -0.17 & -0.04 [-0.69, +0.61] & 0.905 & -0.05 [-0.70, +0.60] & 0.883 \\
Knowledge quiz (0--5) & -0.11 & +0.01 [-0.97, +0.99] & 0.987 & +0.00 [-0.97, +0.98] & 0.994 \\
STEM interest (composite) & -0.01 & +0.14 [-0.49, +0.78] & 0.657 & +0.14 [-0.49, +0.78] & 0.660 \\
SCCT self-efficacy (composite) & +0.03 & +0.12 [-0.37, +0.62] & 0.622 & +0.12 [-0.38, +0.62] & 0.638 \\
Perceived engagement & -1.26 & -1.20 [-1.78, -0.62] & $<0.001$$^{***}$ & -1.20 [-1.78, -0.62] & $<0.001$$^{***}$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/baseline.tex <==
\begin{table}[t]
\centering
\caption{Baseline comparability of the SDT (Sweden) and Control (Italy) groups before the intervention (pre-questionnaire, student sample). Standardised mean differences (SMD) are absolute values; values $\geq 0.50$ (bold) indicate non-negligible imbalance.}
\label{tab:baseline}
\begin{tabular}{lrrrrrrc}
\toprule
Item & SDT $n$ & SDT & Ctrl $n$ & Ctrl & SMD & $p$ \\
\midrule
Age (years, M (SD)) & 61 & 15.18 (0.59) & 19 & 16.21 (0.42) & \textbf{1.85} & $<0.001$$^{***}$ \\
Female (\%) & 62 & 37.1 & 19 & 26.3 & 0.23 & 0.426 \\
Prior robotics experience (\%) & 50 & 50.0 & 19 & 31.6 & 0.38 & 0.189 \\
Prior automatic control experience (\%) & 50 & 20.0 & 19 & 5.3 & 0.41 & 0.268 \\
Prior programming experience (\%) & 50 & 80.0 & 19 & 52.6 & \textbf{0.64} & 0.035$^{*}$ \\
Prior simulator experience (\%) & 50 & 54.0 & 19 & 0.0 & \textbf{1.27} & $<0.001$$^{***}$ \\
Gaming weekdays (median 0--3) & 50 & 0.5 & 19 & 0.0 & 0.42 & 0.146 \\
Gaming weekends (median 0--3) & 50 & 1.0 & 19 & 0.0 & \textbf{0.86} & 0.002$^{**}$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/cmb.tex <==
\begin{table}[t]
\centering\small
\caption{Common-method-bias diagnostics (Harman single-factor test): variance explained by the first unrotated principal component of all 17 Likert items. Values well below the 50\% heuristic indicate that a single common method factor does not dominate the responses.}
\label{tab:cmb}
\begin{tabular}{lrr}
\toprule
Sample & First-factor variance (\%) & $n$ \\
\midrule
Pre-questionnaire (all) & 33.1 & 67 \\
Post-questionnaire (all) & 45.2 & 59 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/fe_models.tex <==
\begin{table}[t]
\centering\small
\caption{Site fixed-effects models (session fixed effects, HC1 robust standard errors). ``Change'' is the pre--post change in the control condition; ``$\Delta\Delta$'' is the additional change in the SDT condition, i.e.\ the site-adjusted between-condition contrast. Session fixed effects absorb all stable site characteristics (country, school, language, workshop format).}
\label{tab:fe}
\begin{tabular}{lrrrr}
\toprule
Outcome & Change (Ctrl) & $\Delta\Delta$ (SDT$-$Ctrl) & $p$ & $n$ \\
\midrule
PID self-efficacy (composite) & +1.16 (0.27) & -0.05 (0.33) & 0.883 & 140 \\
Knowledge quiz (0--5) & +0.26 (0.43) & +0.00 (0.50) & 0.994 & 140 \\
STEM interest (composite) & +0.01 (0.24) & +0.14 (0.32) & 0.660 & 140 \\
SCCT self-efficacy (composite) & +0.53 (0.20) & +0.12 (0.25) & 0.638 & 140 \\
Perceived engagement & +0.89 (0.22) & -1.20 (0.30) & $<0.001$$^{***}$ & 127 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/gender.tex <==
\begin{table}[t]
\centering\small
\caption{Gender $\times$ time interactions with session fixed effects: the coefficient is the additional pre--post change for female relative to male participants (female $-$ male gap in change), adjusting for age and site. Robust (HC1) standard errors. $^{*}p<0.05$, $^{**}p<0.01$, $^{***}p<0.001$.}
\label{tab:gender}
\begin{tabular}{lrrrr}
\toprule
Outcome & Female $-$ male $\Delta$ [95\% CI] & $p$ & $n_F$ (post) & $n$ \\
\midrule
\multicolumn{5}{l}{\textbf{SDT (Sweden)}} \\[1pt]
\quad PID self-efficacy (composite) & -1.06 [-1.80, -0.31] & 0.006$^{**}$ & 20 & 102 \\
\quad Knowledge quiz (0--5) & -0.48 [-1.48, +0.52] & 0.348 & 20 & 102 \\
\multicolumn{5}{l}{\textbf{Control (Italy)}} \\[1pt]
\quad PID self-efficacy (composite) & -0.92 [-1.87, +0.04] & 0.060 & 5 & 38 \\
\quad Knowledge quiz (0--5) & +1.10 [-0.53, +2.73] & 0.185 & 5 & 38 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/knowledge.tex <==
\begin{table}[t]
\centering\small
\caption{Objectively scored knowledge quiz (multiple-choice, 0/1 items). Item-level comparisons use two-proportion $z$-tests with Holm correction within each group; the composite is analysed with Welch's $t$-test. KR-20 = 0.58 (pre), 0.54 (post). $^{*}p<0.05$, $^{**}p<0.01$, $^{***}p<0.001$ (Holm-adjusted).}
\label{tab:knowledge}
\begin{tabular}{lrrrrrrrr}
\toprule
& \multicolumn{4}{c}{SDT (Sweden)} & \multicolumn{4}{c}{Control (Italy)} \\
\cmidrule(lr){2-5}\cmidrule(lr){6-9}
Item & Pre \% & Post \% & $\Delta$pp & $p_{Holm}$ & Pre \% & Post \% & $\Delta$pp & $p_{Holm}$ \\
\midrule
K1 Serious-game definition & 73.3 & 85.4 & +12.0 & 0.751 & 68.4 & 73.7 & +5.3 & 1.000 \\
K2 Purpose of a control system & 83.1 & 85.4 & +2.3 & 1.000 & 63.2 & 57.9 & -5.3 & 1.000 \\
K3 PID acronym & 47.4 & 58.5 & +11.2 & 1.000 & 21.1 & 31.6 & +10.5 & 1.000 \\
K4 PID components & 72.4 & 70.7 & -1.7 & 1.000 & 31.6 & 47.4 & +15.8 & 1.000 \\
K5 Autonomous motion & 71.7 & 68.3 & -3.4 & 1.000 & 47.4 & 47.4 & +0.0 & 1.000 \\
\midrule
& $n$ & $M$ (SD) & $n$ & $M$ (SD) & $\Delta M$ & $g$ & $p$ & \\
\midrule
SDT & 62 & 3.31 (1.40) & 41 & 3.68 (1.37) & +0.38 & +0.27 & 0.179 \\
Control & 19 & 2.32 (1.49) & 19 & 2.58 (1.02) & +0.26 & +0.20 & 0.530 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/l1so.tex <==
\begin{table}[t]
\centering\small
\caption{Leave-one-session-out sensitivity analysis for the SDT (Sweden) group: $\Delta$ and Hedges' $g$ recomputed with each Swedish session removed in turn.}
\label{tab:l1so}
\begin{tabular}{lrrr}
\toprule
Sample & $\Delta M$ & Hedges' $g$ & $p$ \\
\midrule
\multicolumn{4}{l}{\textit{PID self-efficacy (composite)}} \\[1pt]
\quad All sessions & +0.98 & +1.01 & $<0.001$$^{***}$ \\
\quad omit session 01 & +0.99 & +0.99 & $<0.001$$^{***}$ \\
\quad omit session 02 & +1.01 & +0.99 & $<0.001$$^{***}$ \\
\quad omit session 03 & +1.14 & +1.18 & $<0.001$$^{***}$ \\
\quad omit session 04 & +1.04 & +1.14 & $<0.001$$^{***}$ \\
\quad omit session 05 & +0.67 & +0.70 & 0.007$^{**}$ \\
\quad omit session 06 & +1.00 & +1.05 & $<0.001$$^{***}$ \\
\multicolumn{4}{l}{\textit{Knowledge quiz (0--5)}} \\[1pt]
\quad All sessions & +0.38 & +0.27 & 0.179 \\
\quad omit session 01 & +0.14 & +0.11 & 0.608 \\
\quad omit session 02 & +0.55 & +0.41 & 0.063 \\
\quad omit session 03 & +0.17 & +0.12 & 0.588 \\
\quad omit session 04 & +0.49 & +0.35 & 0.104 \\
\quad omit session 05 & +0.35 & +0.23 & 0.314 \\
\quad omit session 06 & +0.57 & +0.41 & 0.065 \\
\multicolumn{4}{l}{\textit{SCCT self-efficacy (composite)}} \\[1pt]
\quad All sessions & +0.55 & +0.70 & 0.002$^{**}$ \\
\quad omit session 01 & +0.56 & +0.68 & 0.002$^{**}$ \\
\quad omit session 02 & +0.58 & +0.72 & 0.004$^{**}$ \\
\quad omit session 03 & +0.56 & +0.69 & 0.005$^{**}$ \\
\quad omit session 04 & +0.62 & +0.82 & $<0.001$$^{***}$ \\
\quad omit session 05 & +0.34 & +0.42 & 0.091 \\
\quad omit session 06 & +0.62 & +0.86 & $<0.001$$^{***}$ \\
\bottomrule
\end{tabular}
\end{table}


==> tables/moderators.tex <==
\begin{table}[t]
\centering\small
\caption{Within-Sweden moderator analyses (sessions 01--06): pre--post change interacted with workshop duration (6\,h vs.\ 3\,h) and facilitator gender, with session fixed effects and individual covariates. These contrasts are free of cross-country confounding.}
\label{tab:moderators}
\begin{tabular}{lrrrr}
\toprule
Outcome & 6\,h vs.\ 3\,h & $p$ & Female vs.\ male fac. & $p$ \\
\midrule
PID self-efficacy (composite) & -0.45 & 0.533 & -0.74 & 0.070 \\
Knowledge quiz (0--5) & +0.24 & 0.709 & +0.87 & 0.120 \\
SCCT self-efficacy (composite) & -0.34 & 0.551 & -0.10 & 0.761 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/multilevel.tex <==
\begin{table}[t]
\centering\small
\caption{Multilevel models with random intercepts for workshop session (students nested in 7 sessions; 5 sessions with post data contribute to the interaction). $\Delta\Delta$ = post $\times$ SDT interaction; $\sigma^2_{site}$ and $\sigma^2_{resid}$ are the session and residual variance components; ICC = intraclass correlation.}
\label{tab:mlm}
\begin{tabular}{lrrrrrr}
\toprule
Outcome & $\Delta\Delta$ (SE) & $p$ & $\sigma^2_{site}$ & $\sigma^2_{resid}$ & ICC & $n$ \\
\midrule
PID self-efficacy (composite) & -0.04 (0.34) & 0.908 & 0.050 & 0.771 & 0.06 & 140 \\
Knowledge quiz (0--5) & +0.04 (0.49) & 0.934 & 0.464 & 1.611 & 0.22 & 140 \\
STEM interest (composite) & +0.10 (0.35) & 0.768 & 0.191 & 0.823 & 0.19 & 140 \\
SCCT self-efficacy (composite) & +0.14 (0.27) & 0.603 & 0.023 & 0.478 & 0.05 & 140 \\
Perceived engagement & -1.21 (0.34) & $<0.001$$^{***}$ & 0.137 & 0.749 & 0.15 & 127 \\
\bottomrule
\end{tabular}
\end{table}


==> tables/open_ended_learned.tex <==
\begin{table}[htbp]
\centering
\caption{Thematic categorisation of open-ended responses to \textit{What is something interesting you learned?} All five Swedish workshops pooled ($N = 41$).}
\label{tab:open_learned}
\begin{tabular}{lrr}
\toprule
\multicolumn{1}{c}{Theme} & \multicolumn{1}{c}{$n$} & \multicolumn{1}{c}{(\%)} \\
\midrule
    PID / control systems concepts & 7 & (17\%) \\
    Programming / how to program & 6 & (15\%) \\
    Robot behaviour / balance mechanisms & 4 & (10\%) \\
    Autonomy / autonomous systems & 1 & (2\%) \\
    Practical / engineering applications & 1 & (2\%) \\
    General STEM / robotics awareness & 3 & (7\%) \\
    Nothing / don't know & 14 & (34\%) \\
    Negative / explicit disinterest & 1 & (2\%) \\
    Meta-reflection on learning & 4 & (10\%) \\
\bottomrule
\end{tabular}
\end{table}


==> tables/open_ended_notworked.tex <==
\begin{table}[htbp]
\centering
\caption{Thematic categorisation of open-ended responses to \textit{What did not work well? Suggestions?} All five Swedish workshops pooled ($N = 41$). Percentages may sum to more than 100\% where individual responses were assigned to more than one thematic category.}
\label{tab:open_notworked}
\begin{tabular}{lrr}
\toprule
\multicolumn{1}{c}{Theme} & \multicolumn{1}{c}{$n$} & \multicolumn{1}{c}{(\%)} \\
\midrule
    Presentation too long / excessive theory & 5 & (12\%) \\
    Technical difficulties (connection, platform) & 8 & (20\%) \\
    Lack of conceptual clarity (PID, instructions) & 3 & (7\%) \\
    Too easy / insufficient challenge & 1 & (2\%) \\
    Too difficult / confusing & 3 & (7\%) \\
    Poor presentation quality / delivery & 3 & (7\%) \\
    Generic negative ("everything") & 3 & (7\%) \\
    Nothing / no issues & 8 & (20\%) \\
    Don't know / non-informative & 5 & (12\%) \\
    Wanted more activities & 1 & (2\%) \\
    Simulator/platform issues & 1 & (2\%) \\
\bottomrule
\end{tabular}
\end{table}


==> tables/open_ended_worked.tex <==
\begin{table}[htbp]
\centering
\caption{Thematic categorisation of open-ended responses to \textit{What worked well during the activity?} All five Swedish workshops pooled ($N = 41$). Percentages may sum to more than 100\% where individual responses were assigned to more than one thematic category.}
\label{tab:open_worked}
\begin{tabular}{lrr}
\toprule
\multicolumn{1}{c}{Theme} & \multicolumn{1}{c}{$n$} & \multicolumn{1}{c}{(\%)} \\
\midrule
    Practical / hands-on activities & 9 & (22\%) \\
    Collaboration / teamwork & 3 & (7\%) \\
    Clear instructions / materials & 3 & (7\%) \\
    Facilitator explanation quality & 2 & (5\%) \\
    Simulator / serious game & 4 & (10\%) \\
    Generic positive ("everything") & 11 & (27\%) \\
    Don't know / non-informative & 4 & (10\%) \\
    Nothing worked well & 3 & (7\%) \\
    Listening to presentation & 2 & (5\%) \\
\bottomrule
\end{tabular}
\end{table}


==> tables/prepost.tex <==
\begin{table}[t]
\centering\small
\caption{Within-group pre--post changes (independent samples, Welch's $t$-test). Top panel: confirmatory outcomes (Holm-corrected within family). Bottom panel: secondary outcomes. $^{*}p<0.05$, $^{**}p<0.01$, $^{***}p<0.001$ (uncorrected).}
\label{tab:prepost}
\begin{tabular}{lrrrrrr}
\toprule
Outcome & SDT pre & Ctrl pre & & $\Delta$ / $g$ & & \\
\midrule
\multicolumn{7}{l}{\textbf{Primary (confirmatory) outcomes}} \\
\multicolumn{7}{l}{\textit{PID self-efficacy (composite)}} \\[1pt]
\quad $M_{pre}$ (SD) & 1.72 (0.79) & 1.53 (0.72) & $\Delta M_{SDT}$ & +0.98$^{***}$ & $\Delta M_{Ctrl}$ & +1.16$^{***}$ \\
\quad Hedges' $g$ & \multicolumn{2}{c}{+1.01} & \multicolumn{2}{c}{+1.25} & $p_{Holm}$ (SDT) & $<0.001$ \\[3pt]
\multicolumn{7}{l}{\textit{Knowledge quiz (0--5)}} \\[1pt]
\quad $M_{pre}$ (SD) & 3.31 (1.40) & 2.32 (1.49) & $\Delta M_{SDT}$ & +0.38 & $\Delta M_{Ctrl}$ & +0.26 \\
\quad Hedges' $g$ & \multicolumn{2}{c}{+0.27} & \multicolumn{2}{c}{+0.20} & $p_{Holm}$ (SDT) & 0.358 \\[3pt]
\multicolumn{7}{l}{\textit{STEM interest (composite)}} \\[1pt]
\quad $M_{pre}$ (SD) & 2.65 (1.05) & 3.28 (0.61) & $\Delta M_{SDT}$ & -0.09 & $\Delta M_{Ctrl}$ & +0.01 \\
\quad Hedges' $g$ & \multicolumn{2}{c}{-0.09} & \multicolumn{2}{c}{+0.02} & $p_{Holm}$ (SDT) & 0.669 \\[3pt]
\midrule
\multicolumn{7}{l}{\textbf{Secondary outcomes}} \\
\multicolumn{7}{l}{\textit{SCCT self-efficacy (composite)}} \\[1pt]
\quad $M_{pre}$ (SD) & 2.71 (0.66) & 2.35 (0.58) & $\Delta M_{SDT}$ & +0.55$^{**}$ & $\Delta M_{Ctrl}$ & +0.53$^{*}$ \\
\quad Hedges' $g$ & \multicolumn{2}{c}{+0.70} & \multicolumn{2}{c}{+0.72} & $p_{Holm}$ (SDT) & 0.008 \\[3pt]
\multicolumn{7}{l}{\textit{Robotics perception (composite)}} \\[1pt]
\quad $M_{pre}$ (SD) & 2.80 (0.67) & 2.51 (0.53) & $\Delta M_{SDT}$ & +0.45$^{**}$ & $\Delta M_{Ctrl}$ & +0.50$^{*}$ \\
\quad Hedges' $g$ & \multicolumn{2}{c}{+0.59} & \multicolumn{2}{c}{+0.74} & $p_{Holm}$ (SDT) & 0.029 \\[3pt]
\multicolumn{7}{l}{\textit{SCCT outcome expectations}} \\[1pt]
\quad $M_{pre}$ (SD) & 3.46 (0.92) & 3.32 (0.50) & $\Delta M_{SDT}$ & -0.10 & $\Delta M_{Ctrl}$ & +0.30 \\
\quad Hedges' $g$ & \multicolumn{2}{c}{-0.11} & \multicolumn{2}{c}{+0.51} & $p_{Holm}$ (SDT) & 1.000 \\[3pt]
\multicolumn{7}{l}{\textit{SCCT contextual support}} \\[1pt]
\quad $M_{pre}$ (SD) & 3.44 (0.78) & 3.24 (0.57) & $\Delta M_{SDT}$ & -0.09 & $\Delta M_{Ctrl}$ & +0.33 \\
\quad Hedges' $g$ & \multicolumn{2}{c}{-0.11} & \multicolumn{2}{c}{+0.52} & $p_{Holm}$ (SDT) & 1.000 \\[3pt]
\multicolumn{7}{l}{\textit{Perceived engagement}} \\[1pt]
\quad $M_{pre}$ (SD) & 3.69 (0.94) & 3.37 (0.68) & $\Delta M_{SDT}$ & -0.35 & $\Delta M_{Ctrl}$ & +0.89$^{***}$ \\
\quad Hedges' $g$ & \multicolumn{2}{c}{-0.35} & \multicolumn{2}{c}{+1.31} & $p_{Holm}$ (SDT) & 0.308 \\[3pt]
\bottomrule
\end{tabular}
\end{table}


==> tables/triangulation.tex <==
\begin{table}[t]
\centering\scriptsize
\caption{Evidence triangulation across three data sources: self-report Likert items, objectively scored knowledge quiz, and qualitatively coded open-ended responses (Swedish workshops, $N=41$).}
\label{tab:triangulation}
\begin{tabular}{p{2.3cm}p{3.3cm}p{3.3cm}p{3.2cm}p{2.0cm}}
\toprule
Construct & Self-report & Objective knowledge & Qualitative themes & Verdict \\
\midrule
\textit{PID controller competence} & SDT $g=+1.01$; Ctrl $g=+1.25$ & K3 +11/+11 pp; K4 -2/+16 pp & ``PID/control concepts'' cited by 7/41 (17\%) as learning outcome & Mostly convergent (objective mixed) \\
\textit{Control-system understanding} & SDT $g=+0.55$; Ctrl $g=+0.57$ & K2 +2/-5 pp & ``Programming/how to program'' 6/41 (15\%); robot balancing 4/41 (10\%) & Partly convergent \\
\textit{Basic robotics} & SDT $g=+0.53$; Ctrl $g=+0.32$ & K5 -3/+0 pp; K1 +12/+5 pp & ``Practical/hands-on'' 9/41 (22\%) as strongest element & Convergent (self-report and qualitative), less so objectively \\
\textit{STEM interest and career plans} & SDT $g=-0.09$ (ns); Ctrl $g=+0.02$ (ns) & No knowledge item targets career interest & No career-interest theme; occasional disinterest (1/41) & Convergent null \\
\bottomrule
\end{tabular}
\end{table}

